Building DNN Acoustic Models for Large Vocabulary Speech Recognition

Deep neural networks (DNNs) are now a central component of nearly all state-of-the-art speech recognition systems. Building neural network acoustic models requires several design decisions including network architecture, size, and training loss function. This paper offers an empirical investigation on which aspects of DNN acoustic model design are most important for speech recognition system performance. We report DNN classifier performance and final speech recognizer word error rates, and compare DNNs using several metrics to quantify factors influencing differences in task performance. Our first set of experiments use the standard Switchboard benchmark corpus, which contains approximately 300 hours of conversational telephone speech. We compare standard DNNs to convolutional networks, and present the first experiments using locally-connected, untied neural networks for acoustic modeling. We additionally build systems on a corpus of 2,100 hours of training data by combining the Switchboard and Fisher corpora. This larger corpus allows us to more thoroughly examine performance of large DNN models -- with up to ten times more parameters than those typically used in speech recognition systems. Our results suggest that a relatively simple DNN architecture and optimization technique produces strong results. These findings, along with previous work, help establish a set of best practices for building DNN hybrid speech recognition systems with maximum likelihood training. Our experiments in DNN optimization additionally serve as a case study for training DNNs with discriminative loss functions for speech tasks, as well as DNN classifiers more generally.

==> dnn_analysis.tex <==
\section{Analyzing Trained DNNs}\label{sec:analysis_dnn}
This section compares the coding properties of DNNs to better
understand what aspects of DNN representations lead to differences in
performance.

XXX

\subsection{Sparsity and Dispersion}
XXX scree plots for models of various size

TODO need publication quality plots made for these


\subsection{Eigenvalue Representation Analysis}
TODO still unclear if this is a useful analysis tool


\section{Comparing Phone Classification and WER Across Models}
TODO looking back at these plots I'm not sure there is much of a conclusion to discuss here. 


==> experiment_fisher.tex <==
\subsection{Fisher 2,000 Hour Corpus}\label{sec:experiment_fisher}
On the Switchboard 300 hour corpus we observed limited benefits from
increasing DNN model size for acoustic modeling, even with a variety
of techniques to improve generalization performance. We next explore
the impact of DNN model size on a much larger speech corpus than
Switchboard, the Fisher 2,000 hour conversational speech corpus
\cite{Cieri2004Fisher}. The Fisher corpus contains 23,394 unique
speakers compared to the 4,870 unique speakers in our Switchboard
training set. Like Switchboard, Fisher speech comes from two-party
telephone conversations of roughly ten minutes in length on a directed
topic. However, Fisher uses semi-automated transcriptions which are
slightly lower in quality as compared to the Switchboard
transcriptions.

We built a separate baseline HMM-GMM system using a nearly identical
training recipe as that used in our Switchboard system. Although it is
possible to build a substantially better HMM-GMM baseline with the
increased amount of training data, we kept the number HMM states
roughly equivalent to that of our Switchboard baseline. Our Fisher GMM
baseline recognizer has 7,793 sub-phone states and 300K Gaussians. We
build a language model using only the Fisher transcripts without
additional text resources. For all DNN models we use a context window
of +/- 10 frames. To evaluate performance on the Fisher corpus we hold
out a speaker-disjoint set of 5,000
utterances. Table~\ref{tab:res_fisher} shows the performance of our
baseline system on the Fisher evaluation set as well as the Hub5
evaluation sets to compare against our Switchboard-trained
systems. Our Fisher baseline system performs comparably to our
Switchboard baseline system (see Table~\ref{tab:res_nonlin}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Note use of \abovespace and \belowspace to get reasonable spacing 
% above and below tabular lines. 
\begin{table*}[bth]
\caption{Results for baseline and DNN systems trained on the Fisher
  corpus. We evaluate word error rate and frame-level metrics on a
  speaker held-out subset of the Fisher corpus (FSH). For comparison we
  additionally evaluate models trained on Fisher using the same Hub5
  2000 evaluation sets used in Table~\ref{tab:res_nonlin}. We train
  models using a 300 hour Fisher subset and the full 2,000 hour
  corpus. All DNNs have 5 hidden layers with either 2,048 hidden units
  (36M parameters) or 5,984 hidden units (200M parameters).}
\label{tab:res_fisher}
%\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{lllrrrrrr }
\toprule
Model & Train Hours & Dev CrossEnt & Dev Acc(\%) & SWBD WER & CH WER 
& EV WER & FSH WER\\
\midrule
GMM & 2000 & N/A & N/A & 24.3 & 33.9 & 29.3 & 32.3\\
\midrule
2048 Layer (36M) & 300 & 2.23 & 49.9 & 18.0 & 26.1 & 22.1 & 24.2\\
2048 Layer (36M) & 2000 & 1.99 & 53.1 & 17.1 & 25.1 & 21.1 & 23.3\\
\midrule
5984 Layer (200M) & 300 & 2.34 & 49.8 & 17.5 & 25.5 & 21.7 & 23.7\\
5984 Layer (200M) & 2000 & 1.91 & 55.1 & 16.0 & 23.7 & 19.9 & 21.9\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We test the effect of training on more data by building DNN acoustic
models for the full 2,000 hour dataset as well as a 300 hour subset of
the training data. Our 300 hour training subset does not randomly
sample from all speakers in the full training set. Instead, we
construct 300 hours of data by adding all data for a speaker until the
total number of hours reaches 300. Constructing training subsets in
this way controls for the beneficial effects of observing large
numbers of speakers. For both training set sizes, we train a DNN with
5 hidden layers of 5,984 hidden units for a total of 200M parameters.
We additionally train baseline DNNs with 5 layers of 2,048 hidden
units for a total of 36M parameters. DNN training uses the same
procedure described in Section~\ref{sec:experiment_swbd}.
Table~\ref{tab:res_fisher} shows WER and frame-level
performance metrics for DNNs trained on the Fisher corpus.

With 36M parameter DNN acoustic models, increasing the training set
size from 300 to 2,000 hours produces a significant gain on all WER
evaluation sets. This DNN is of a scale representative of most DNN
acoustic models used in practice. Our results suggest DNNs of even
modest size improve performance when leveraging the larger 2,000 hour
training set. We note that neither 36M parameter model trained on the
Fisher corpus outperforms a 36M parameter DNN trained on Switchboard
when evaluating in terms of the Switchboard evaluation sets. This is
not surprising as training and testing on Switchboard presents a
matched evaluation condition which facilitates generalization. To
facilitate comparison across training corpora, we include results from
our Switchboard systems on the Fisher evaluation set in
Table~\ref{tab:res_nonlin}. We find that while the baseline GMM
systems perform somewhat comparably across corpora, results from
mismatched evaluation conditions are always worse.


With the Fisher corpus we observe significant gains from increasing
the acoustic model size from 36M to 200M total parameters. On the
Fisher evaluation set our 200M model achieves a 1.3\% absolute
reduction in WER from the 36M parameter model when both are trained on
the full 2,000 hour corpus. However, when comparing across model sizes
for DNNs trained on the 300 hour subset we find a much smaller gain of
0.6\% from increasing DNN model size. Again this suggests that a large
training corpus is necessary to fully take advantage of the
capabilities of large DNNs for acoustic modeling. Our large DNN
trained on the full Fisher corpus achieves a 0.7\% absolute reduction
in WER on the full Hub5 evaluation set over our best
Switchboard-trained systems. Although Fisher data differs slightly
from Switchboard, increasing model training set sizes provides a more
direct path to performance improvements as compared to generalization 
techniques like dropout. It is also important to note that
frame-level performance is substantially lower for Fisher corpus
models as compared with Switchboard models. The low frame-level
performance of even our 200M parameter model suggests there is still
room to improve by increasing DNN model size to better fit the
available training data.



==> related_work.tex <==
\section{Related Work}\label{sec:related_work}
Using neural networks as acoustic models for HMM-based speech
recognition was introduced over 20 years ago
\cite{Bourlard93,Renals1994,McClelland1986}. Much of this original work
developed the basic ideas of hybrid HMM-DNN systems which are used in
modern, state-of-the-art systems. However, until much more recently
neural networks were not a standard component in the highest
performing LVCSR systems. Computational constraints and the amount of
available training data severely limited the pace at which it was
possible to make progress on neural network research for speech
recognition.
Instead, Gaussian mixture models were the standard choice for
acoustic modeling as researchers worked to refine the HMM
architecture, decoding frameworks, and signal processing challenges
associated with building high-performance speech recognizers. 

As other aspects of speech recognition systems become more
standardized, it became clear that acoustic models were the source of
many errors in LVCSR systems. As a response, researchers developed
increasingly complex variants to extend the capabilities of GMM
acoustic models to more challenging datasets. Techniques of this type
include subspace GMMs \cite{Povey2011} and semi-tied covariance GMMs
\cite{Gales1999}. An alternative approach to making acoustic models
more expressive is training HMM-GMM systems with discriminative loss
functions, for example the maximum mutual information loss function
\cite{Bahl1986}. Discriminative loss functions, as compared with
standard maximum likelihood training, better focus the limited
representational capacity of the acoustic model on fixing errors which
most impact final system performance.

While GMMs and their extensions produced gains on benchmark LVCSR
tasks over the span of many years, the resulting systems became
increasingly complex. Many of the complexities introduced focused
purely on increasing the representational capacity of GMM acoustic
models. In parallel to this effort, neural networks started to undergo
a resurgence of interest in the machine learning community under the
new branding of \emph{deep learning}. Work in this area focused on
overcoming optimization issues involved in training DNNs. Early papers
in this line of work focused on initializing the weights of a DNN
layer by layer using an unsupervised loss function
\cite{Hinton2006a,Hinton2006b,Vincent2010}. DNNs provided an
interesting path forward for acoustic modeling as neural networks
offer a direct path to increasing representational capacity, provided
it is possible to find a good set of DNN parameters. Early experiments
with DNNs used fairly small phoneme recognition tasks, but in 2011
researchers used a pre-trained DNN on a large vocabulary speech task
and obtained a large reduction in WER \cite{Dahl2011,Jaitly2012}.

The initial success of DNN acoustic models as compared with existing
GMM acoustic models resulted in quick adoption across a range of
research groups and speech recognition tasks
\cite{Hinton2013}. Indeed, speech recognition was one of the early,
clear successes produced by modern DNN research. DNN acoustic models
are now part of many of the highest-performing systems for languages
where sufficient training data is available. Several groups found
that, due to the abundance of labeled data available when training DNN
acoustic models, the unsupervised pre-training step is not necessary.

In recent years, the speech recognition research community has focused
a significant research effort on both improving DNN acoustic models
applying DNNs to other tasks related to speech recognition. The
discriminative loss functions used to train GMM acoustic models were
adapted to train DNNs, yielding small gains for DNNs which are first
trained with the standard cross entropy loss function
\cite{Povey2013,Kingsbury2012,Seide2013}. In addition to modifying the
loss function for acoustic model training, there has been work on
alternative neural network architectures for speech
recognition. Recent work with DCNNs found them to be useful first on
phoneme recognition tasks but also on LVCSR tasks when used in
addition to a standard DNN acoustic model
\cite{AbdelHamid2012,Sainath2013,Sainath2014}. Other work focuses on
modern approaches to 
recurrent network structures to better leverage the temporal structure
of speech signals for acoustic modeling \cite{Robinson1991,Graves2013,Sak2014}
Standard DNNs have
also undergone modification, as several groups found replacing the
standard sigmoidal hidden units with rectified linear units in DNNs
leads to WER gains and simpler training procedures
\cite{Dahl2013,Zeiler2013,Maas2013}.
Within the broader field of spoken language processing there is a
resurgence of interest in applying neural networks to existing tasks
including language modeling, noise reduction, and speaker recognition
\cite{Campbell2014,Maas2012,Mikolov2010}. Indeed, wherever there is a
task requiring supervised classification or regression techniques
neural networks are often tested and successful as compared to
previous, simpler prediction techniques.


XXX

Note that it is possible to use neural network outputs as features for
an HMM-GMM system using a \emph{tandem} recognition approach.


%% CNN:

%% % TODO Cite LeCun, Imagenet results?
%% % TODO May want to move some  of this into Related Work
%% While fully-connected DNNs have been adopted as the primary neural network architecture
%% for HMM acoustic models,
%% recently work has shown improved results using deep convolutional neural
%% networks (DCNNs) in place of fully-connected DNNs in
%% large hybrid HMM systems.
%% DCNNs have achieved state-of-the-art results across a wide range of tasks
%% in the computer vision community, and have been applied to natural language
%% processing tasks as well \cite{LeCun1998, Krizhevsky2012, Collobert2011b}.
%% Proponents of DCNN acoustic models argue that DCNNs allow for parameter sharing
%% and exploit local correlations along the frequency and
%% time domains. Pooling further helps with small shifts and speaker variations in
%% the speech signal.
%% DCNN acoustic models have obtained gains in word error rate on smaller datasets
%%  such as TIMIT 
%% as well as for a larger 400 hour broadcast news dataset and the 300 hour Switchboard dataset
%% \cite{Sainath2013, Sainath2014}.

%% DCNN acoustic models have obtained
%% gains in word error rate on smaller datasets such as TIMIT
%% \cite{AbdelHamid2012}, as well as for a larger 400 hour broadcast news
%% dataset and the 300 hour Switchboard dataset \cite{Sainath2013,
%%   Sainath2014}.

%% XXX rewrite:

%% Researchers invented alternative loss functions for acoustic model
%% training that re-weight training samples to focus attention on samples
%% which most impact final system WER. Specific loss functions of this
%% form include maximum mutual information (MMI) and minimum Bayes risk
%% (MBR) \cite{Povey2013}. Such loss functions were historically
%% important because Gaussian mixture model (GMM) acoustic models have
%% limited representational capacity. When representational power is
%% limited, focusing on samples that most affect WER is important. MMI and
%% similar loss functions can also yield small gains on top of cross
%% entropy training of DNN acoustic models. Such loss functions help
%% limited capacity, small DNN models focus on the appropriate
%% samples. In this work we employ DNNs which fit training samples
%% substantially better than the smaller DNNs of previous work.


